Deliberated Domain Bridging for Domain Adaptive Semantic Segmentation

In unsupervised domain adaptation (UDA), directly adapting from the source to the target domain usually suffers significant discrepancies and leads to insufficient alignment. Thus, many UDA works attempt to vanish the domain gap gradually and softly via various intermediate spaces, dubbed domain bridging (DB). However, for dense prediction tasks such as domain adaptive semantic segmentation (DASS), existing solutions have mostly relied on rough style transfer and how to elegantly bridge domains is still under-explored. In this work, we resort to data mixing to establish a deliberated domain bridging (DDB) for DASS, through which the joint distributions of source and target domains are aligned and interacted with each in the intermediate space. At the heart of DDB lies a dual-path domain bridging step for generating two intermediate domains using the coarse-wise and the fine-wise data mixing techniques, alongside a cross-path knowledge distillation step for taking two complementary models trained on generated intermediate samples as 'teachers' to develop a superior 'student' in a multi-teacher distillation manner. These two optimization steps work in an alternating way and reinforce each other to give rise to DDB with strong adaptation power. Extensive experiments on adaptive segmentation tasks with different settings demonstrate that our DDB significantly outperforms state-of-the-art methods. Code is available at https://github.com/xiaoachen98/DDB.git.

==> figure/overview.tex <==
\begin{figure*}[t]
    \centering
    \scalebox{0.6}{\includegraphics{figure/fig_file/fig1/overview.pdf}}
    \captionsetup{font={footnotesize}}
    \caption{\textbf{Illustration of domain bridging based (a) \emph{Baseline} and (b) our proposed \emph{PLDB}.} (a) \emph{Baseline} (e.g., CyCADA []) employs CycleGAN [] based techniques to create an intermediate domain that appears to be closer to the target domain, facilitating knowledge transfer. (b) Our proposed \emph{PLDB} construct bridges over the cross-domain joint distributions. Specifically, we utilize distinct spatial space-based domain bridging methods to construct dual-path domain bridging (DDB) on the complementary region-path and class-path. Furthermore, the cross-path distillation (CKD) is designed to integrate knowledge from the complementary teachers to a student. After alternating rounds of DDB and CKD, the knowledge will be progressively learned and transferred.}
    \label{fig:1}
\end{figure*}

==> figure/overview_new.tex <==
\begin{figure*}[t]
    \centering
    \scalebox{0.54}{\includegraphics{figure/fig_file/fig1/overview_new.pdf}}
    \captionsetup{font={footnotesize}}
    \caption{\textbf{Illustration of various domain bridging approaches on domain adaptive semantic segmentation.} (a) Style transfer-based methods employ various style transfer \cite{zhu2017unpaired,reinhard2001color} techniques to create an intermediate domain in the input space that appears to be closer to the target domain. (b) Global blending-based methods employ pixel-wise Mixup \cite{zhang2018mixup} technique to globally construct an intermediate domain in the input and label space. On the contrary, (c) and (d) would regionally construct an intermediate domain in the input and label space. (c) Coarse region-based methods aim to randomly copy a regular \cite{yun2019cutmix} or irregular \cite{harris2020fmix,french2020milking} region from the source domain and paste it to the target domain. (d) Fine region-based methods \cite{olsson2021classmix,zhou2021context} utilize the annotation in the source domain to randomly select fine region of classes and paste it to the target domain.
    }
    \label{fig:1}
\end{figure*}

==> figure/shift_confusion.tex <==
\begin{figure*}[t]
    \centering
    \hspace{-2pt}
    \captionsetup{font={footnotesize}}
    \includegraphics[width=0.9\textwidth]{figure/fig_file/shift_confusion_new.pdf}\\
    \vspace{-2pt}
    \caption{Qualitative results of coarse region-path (CRP) and fine region-path (FRP) bridging methods on the GTA5~$\to$~Cityscapes benchmark. }
    \label{fig:2}
\end{figure*}

==> figure/umap.tex <==
\begin{wrapfigure}{r}{0.6\textwidth}
\vspace{-10.5pt}
\centering
\captionsetup{font={footnotesize}}
\vspace{-2pt}
\subfloat[Source only]{\includegraphics[width=0.49\linewidth,height=0.08\textheight]{figure/fig_file/source_only.pdf}}
\subfloat[Coarse region-path]{\includegraphics[width=0.49\linewidth,height=0.08\textheight]{figure/fig_file/cutmix.pdf}} \\
\subfloat[Final model]{\scalebox{-1}[-1]{\includegraphics[width=0.49\linewidth,height=0.08\textheight]{figure/fig_file/ckd_r2.pdf}}}
\subfloat[Fine region-path]{\scalebox{-1}[1]{\includegraphics[width=0.49\linewidth,height=0.08\textheight]{figure/fig_file/classmix.pdf}}}
\caption{We use UMAP [] to visualize the feature space obtained before the classification layer. For a clear analysis, we select two pairs of categories that suffer from labeling shift and confusion, respectively, \emph{i.e.}, salmon for `road', spring green for `sidewalk', slate gray for `bus', and slate blue for `train'}
\label{fig:3}
\end{wrapfigure}

==> figure/umap_full_line.tex <==
\begin{figure*}[t]
    \vspace{-10.5pt}
    \centering
    \captionsetup{font={footnotesize}}
    \vspace{-2pt}
    \subfloat[Source only]{\includegraphics[width=0.245\textwidth,height=0.12\textheight]{figure/fig_file/source_only.pdf}}
    \subfloat[Coarse region-path]{\includegraphics[width=0.245\textwidth,height=0.12\textheight]{figure/fig_file/cutmix.pdf}}
    \subfloat[Fine region-path]{\scalebox{-1}[1]{\includegraphics[width=0.245\textwidth,height=0.1\textheight]{figure/fig_file/classmix.pdf}}}
    \subfloat[Final model]{\scalebox{-1}[-1]{\includegraphics[width=0.245\textwidth,height=0.1\textheight]{figure/fig_file/ckd_r2.pdf}}}
    \caption{UMAP \cite{mcinnes2018umap} visualization of the feature space before the classification layer on GTA5~$\to$~Cityscapes. For a clear analysis, we select two pairs of categories that suffer from labeling shift and confusion, respectively, \emph{i.e.}, salmon for road, spring green for sidewalk, slate gray for bus, and slate blue for train.}    
    \label{fig:3}
\end{figure*}

==> table/ablation.tex <==
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}} 
\begin{wraptable}{rt}{0.5\linewidth}
    \centering
    \captionsetup{font={scriptsize}}
    \vspace{-11.5pt}
    \captionof{table}{Ablation study of each proposed component on the GTA5~$\to$~Cityscapes benchmark. The teacher models in the next round of DDB are loaded with the weights from the student model obtained from previous round of CKD .}
    \setlength\tabcolsep{1.6pt}{
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{@{}c|ccc|ll@{}}
        \toprule
        &\multicolumn{3}{c|}{components} &\multicolumn{1}{l}{mIoU} & \multicolumn{1}{l}{gain}\\
        \midrule
        
        &\multicolumn{3}{c|}{source only}
        &\multicolumn{1}{l}{~32.1} &\\
        \midrule
        
        \multirow{4}{*}{\tabincell{c}{stage 1\\DDB}} &\tabincell{c}{self\\training} &\tabincell{c}{region\\path}
        &\tabincell{c}{class\\path}
        &\multicolumn{1}{l}{mIoU} 
        &\multicolumn{1}{l}{gain}\\
        \cline{2-6} 
        
        &\checkmark & & &33.8 &+1.7\\
        &\checkmark &\checkmark & &56.5 &+24.4\\
        &\checkmark & &\checkmark &58.2 &+26.1\\
        \midrule
        
        \multirow{6}{*}{\tabincell{c}{stage 1\\CKD}} &\tabincell{c}{augment\\$x_t$}
        &\tabincell{c}{hard\\distillation}
        &\tabincell{c}{adaptively\\ensemble}
        &\multicolumn{1}{l}{mIoU} 
        &\multicolumn{1}{l}{gain}\\
        \cline{2-6}
        
        & & & &57.0 &+24.9\\
        &\checkmark & & &57.8 &+25.7\\
        &\checkmark &\checkmark & &59.9 &+27.8\\
        &\checkmark & &\checkmark &60.1 &+28.0\\
        &\checkmark &\checkmark &\checkmark &61.2 &+29.1\\
        \midrule
        
        \multirow{3}{*}{\tabincell{c}{stage 2\\DDB}} &\tabincell{c}{self\\training} &\tabincell{c}{region\\path}
        &\tabincell{c}{class\\path}
        &\multicolumn{1}{l}{mIoU} 
        &\multicolumn{1}{l}{gain}\\
        \cline{2-6}
        
        &\checkmark &\checkmark & &61.4 &+29.3\\
        &\checkmark & &\checkmark &62.6 &+30.5\\
        \midrule   
        
        \multirow{1}{*}{\tabincell{c}{stage 2\\CKD}} &\tabincell{c}{augment\\$x_t$}
        &\tabincell{c}{hard\\distillation}
        &\tabincell{c}{adaptively\\ensemble}
        &\multicolumn{1}{l}{mIoU} 
        &\multicolumn{1}{l}{gain}\\
        \cline{2-6}    
        
        &\checkmark &\checkmark &\checkmark &62.7 &+30.6\\
        \toprule
    \end{tabular}}}
    \label{tab:6}
\end{wraptable}

==> table/ablation_all.tex <==
\begin{table}[!t]
	\vspace{10pt}
	\setlength{\fboxrule}{0pt}
	\captionsetup{font={footnotesize}}
	\caption{Ablation studies on three benchmarks.}
	\vspace{-10pt}
	\begin{center}
		\begin{subtable}[ht]{0.32 \textwidth}
		    \begin{center}
		        \captionsetup{font={scriptsize}}
		        \caption{Ablation studies on G~$\to$~C.}
		        \vspace{-4pt}
		        \setlength{\tabcolsep}{2mm}
                \resizebox{0.9\textwidth}{!}{
                    \setlength\tabcolsep{1.6pt}{
                    \begin{tabular}{@{}c|cc|ll}
                        \toprule
                        &\multicolumn{2}{c|}{components} &\multicolumn{1}{l}{mIoU} & \multicolumn{1}{l}{gain}\\
                        \midrule
                        
                        &\multicolumn{2}{c|}{source only}
                        &\multicolumn{1}{l}{~32.1} &\\
                        \midrule
                        
                        \multirow{4}{*}{\tabincell{c}{stage 1\\DDB}}  &\tabincell{c}{region\\path}
                        &\tabincell{c}{class\\path}
                        &\multicolumn{1}{l}{mIoU} 
                        &\multicolumn{1}{l}{gain}\\
                        \cmidrule{2-5} 
                        
                        &\checkmark & &56.5 &+24.4\\
                        & &\checkmark &58.2 &+26.1\\
                        \midrule
                        
                        \multirow{6}{*}{\tabincell{c}{stage 1\\CKD}}
                        &\tabincell{c}{hard\\distillation}
                        &\tabincell{c}{adaptive\\ensemble}
                        &\multicolumn{1}{l}{mIoU} 
                        &\multicolumn{1}{l}{gain}\\
                        \cmidrule{2-5}
                        
                        & & &59.0 &+26.9\\
                        &\checkmark  & &59.9 &+27.8\\
                        & &\checkmark  &61.1 &+29.0\\
                        &\checkmark &\checkmark &61.2 &+29.1\\
                        \midrule
                        
                        \multirow{4}{*}{\tabincell{c}{stage 2\\DDB}} &\tabincell{c}{region\\path}
                        &\tabincell{c}{class\\path}
                        &\multicolumn{1}{l}{mIoU} 
                        &\multicolumn{1}{l}{gain}\\
                        \cmidrule{2-5}
                        
                        &\checkmark & &61.4 &+29.3\\
                        & &\checkmark &62.6 &+30.5\\
                        \midrule   
                        
                        \multirow{3}{*}{\tabincell{c}{stage 2\\CKD}}
                        &\tabincell{c}{hard\\distillation}
                        &\tabincell{c}{adaptive\\ensemble}
                        &\multicolumn{1}{l}{mIoU} 
                        &\multicolumn{1}{l}{gain}\\
                        \cmidrule{2-5}    
                        
                        &\checkmark &\checkmark &62.7 &+30.6\\
                        \toprule
                    \end{tabular}}}
		    \end{center}
		\end{subtable}
		\hspace{3pt}
		\begin{subtable}[ht]{0.32 \textwidth}
		    \begin{center}
		        \captionsetup{font={scriptsize}}
		        \caption{Ablation studies on G~+~S~$\to$~C.}
		        \vspace{-4pt}
		        \setlength{\tabcolsep}{2mm}
                \resizebox{0.9\textwidth}{!}{
                    \setlength\tabcolsep{1.6pt}{
                    \begin{tabular}{@{}c|cc|ll}
                        \toprule
                        &\multicolumn{2}{c|}{components} &\multicolumn{1}{l}{mIoU} & \multicolumn{1}{l}{gain}\\
                        \midrule
                        
                        &\multicolumn{2}{c|}{source only}
                        &\multicolumn{1}{l}{~50.9} &\\
                        \midrule
                        
                        \multirow{4}{*}{\tabincell{c}{stage 1\\DDB}}  &\tabincell{c}{region\\path}
                        &\tabincell{c}{class\\path}
                        &\multicolumn{1}{l}{mIoU} 
                        &\multicolumn{1}{l}{gain}\\
                        \cmidrule{2-5} 
                        
                        &\checkmark & &66.2 &+15.3\\
                        & &\checkmark &66.7 &+15.8\\
                        \midrule
                        
                        \multirow{3}{*}{\tabincell{c}{stage 1\\CKD}}
                        &\tabincell{c}{hard\\distillation}
                        &\tabincell{c}{adaptive\\ensemble}
                        &\multicolumn{1}{l}{mIoU} 
                        &\multicolumn{1}{l}{gain}\\
                        \cmidrule{2-5}
                        
                        % & & &- &-\\
                        % &\checkmark  & &- &-\\
                        % & &\checkmark  &- &-\\
                        &\checkmark &\checkmark &68.6 &+17.7\\
                        \midrule
                        
                        \multirow{4}{*}{\tabincell{c}{stage 2\\DDB}} &\tabincell{c}{region\\path}
                        &\tabincell{c}{class\\path}
                        &\multicolumn{1}{l}{mIoU} 
                        &\multicolumn{1}{l}{gain}\\
                        \cmidrule{2-5}
                        
                        &\checkmark & &68.7 &+17.8\\
                        & &\checkmark &69.0 &+18.1\\
                        \midrule   
                        
                        \multirow{3}{*}{\tabincell{c}{stage 2\\CKD}}
                        &\tabincell{c}{hard\\distillation}
                        &\tabincell{c}{adaptive\\ensemble}
                        &\multicolumn{1}{l}{mIoU} 
                        &\multicolumn{1}{l}{gain}\\
                        \cmidrule{2-5}    
                        
                        &\checkmark &\checkmark &69.0 &+18.1\\
                        \toprule
                    \end{tabular}}}
		    \end{center}
		\end{subtable}
		\hspace{3pt}
		\begin{subtable}[ht]{0.32 \textwidth}
		    \begin{center}
		        \captionsetup{font={scriptsize}}
		        \caption{Ablation studies on G~$\to$~C~+~M.}
		        \vspace{-4pt}
		        \setlength{\tabcolsep}{2mm}
                \resizebox{\textwidth}{!}{
                    \setlength\tabcolsep{1.6pt}{
                    \begin{tabular}{@{}c|cc|llll}
                        \toprule
                        &\multicolumn{2}{c|}{components} &\multicolumn{1}{l}{target} &\multicolumn{1}{l}{mIoU}& \multicolumn{1}{l}{Avg.} & \multicolumn{1}{l}{gain}\\
                        \midrule
                        
                        &\multicolumn{2}{c|}{ \multirow{2}{*}{Source only}}
                        &C &30.1 &\multirow{2}{*}{32.8} &\multirow{2}{*}{} \\
                        && &M &35.5\\
                        \midrule
                        
                        \multirow{6}{*}{\tabincell{c}{stage 1\\DDB}}  &\tabincell{c}{region\\path}
                        &\tabincell{c}{class\\path}
                        &\multicolumn{1}{l}{target} &\multicolumn{1}{l}{mIoU}& \multicolumn{1}{l}{Avg.} & \multicolumn{1}{l}{gain}\\
                        \cmidrule{2-7} 
                        
                        &\checkmark & &\tabincell{l}{C\\M} &\tabincell{l}{51.4\\52.2} &51.8 &+19.0\\
                        & &\checkmark &\tabincell{l}{C\\M} &\tabincell{l}{56.1\\50.4} &53.2 &+20.4\\
                        \midrule
                        
                        \multirow{4}{*}{\tabincell{c}{stage 1\\CKD}}
                        &\tabincell{c}{hard\\distillation}
                        &\tabincell{c}{adaptive\\ensemble}
                        &\multicolumn{1}{l}{target} &\multicolumn{1}{l}{mIoU}& \multicolumn{1}{l}{Avg.} & \multicolumn{1}{l}{gain}\\
                        \cmidrule{2-7}
                        
                        &\checkmark &\checkmark &\tabincell{l}{C\\M} &\tabincell{l}{58.3\\56.5} &57.4 &+24.6\\
                        \midrule
                        
                        \multirow{6}{*}{\tabincell{c}{stage 2\\DDB}} &\tabincell{c}{region\\path} &\tabincell{c}{class\\path}
                        &\multicolumn{1}{l}{target} &\multicolumn{1}{l}{mIoU}& \multicolumn{1}{l}{Avg.} & \multicolumn{1}{l}{gain}\\
                        \cmidrule{2-7}
                        
                        &\checkmark & &\tabincell{l}{C\\M} &\tabincell{l}{59.0\\56.8} &57.9 &+25.1\\
                        & &\checkmark &\tabincell{l}{C\\M} &\tabincell{l}{59.1\\56.7} &57.8 &+25.0\\
                        \midrule   
                        
                        \multirow{4}{*}{\tabincell{c}{stage 2\\CKD}}
                        &\tabincell{c}{hard\\distillation}
                        &\tabincell{c}{adaptive\\ensemble}
                        &\multicolumn{1}{l}{target} &\multicolumn{1}{l}{mIoU}& \multicolumn{1}{l}{Avg.} & \multicolumn{1}{l}{gain}\\
                        \cmidrule{2-7}    
                        
                        &\checkmark &\checkmark &\tabincell{l}{C\\M} &\tabincell{l}{60.4\\56.9} &58.6 &+25.8\\
                        \toprule
                    \end{tabular}}}
		    \end{center}
		\end{subtable}		
	\end{center}
	\vspace{-5pt}
	\label{tab:8}
\end{table}

==> table/complementarity.tex <==
\begin{wraptable}{rt}{0.5\linewidth}
    \centering
    \captionsetup{font={scriptsize}}
    \vspace{-11.5pt}
    \captionof{table}{Comparison results of ensembled models from single path and distinct paths in terms of mIoU. $\mathcal{M}_R^1$ denotes the first run for the region-path model. The best score is indicated in \underline{\textbf{underlined bold}}.}
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{c|cccc}
         \toprule
         & $\mathcal{M}_C^1$ & $\mathcal{M}_C^2$ & $\mathcal{M}_R^1$ & $\mathcal{M}_R^2$ \\
         \midrule
         \vspace{4pt}
         $\mathcal{M}_C^1$ &55.5 &- &- &-\\
         \vspace{4pt}
         $\mathcal{M}_C^2$ &55.9 &55.8 &- &-\\
         \vspace{4pt}
         $\mathcal{M}_R^1$ &56.4 &\textbf{56.8} &55.0 &-\\
         $\mathcal{M}_R^2$ &56.2 &56.6 &55.7 &54.7\\
         \bottomrule
    \end{tabular}}
    \label{tab:5}
\end{wraptable}

==> table/rounds.tex <==
\begin{wraptable}{rt}{0.5\linewidth}
    \centering
    \captionsetup{font={scriptsize}}
    \vspace{-11.5pt}
    \captionof{table}{Performance comparison (mIoU) of the student model obtained from CKD during various rounds in the whole training process on three benchmarks. The best score is indicated in \underline{\textbf{underlined bold}}.}
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{c|cccc}
        \toprule
        &0 &1 &2 &3\\
        \midrule
        G~$\to$~C & 32.3 &61.2 &\underline{\textbf{62.7}} &\underline{\textbf{62.7}}\\
        
        G~+~S~$\to$~C &50.9 &\underline{\textbf{67.4}} &67.1 &-\\
        
        G~$\to$~C~+~M &32.8 &57.4 &\underline{\textbf{58.6}} &\todo{todo}\\
        \bottomrule
    \end{tabular}}
\end{wraptable}
